Zero-Inflated Poisson Cluster-Weighted Models: Properties and Applications

In this paper, I propose a new class of Zero-Inflated Poisson models into the family of Cluster Weighted Models (CWMs) called Zero-Inflated Poisson CWMs (ZIPCWM). ZIPCWM extends Poisson cluster weighted models and other mixture models. I propose an Expectation-Maximization (EM) algorithm via an iteratively reweighted least squares for the model. I theoretically and analytically investigate the identifiability of the proposed model through an extensive simulation study. Parameter recovery, classification assessment, and performance of different information criteria are investigated through broad simulation design. ZIPCWM is applied to real data which accounts for excess zeros of over $40\%$. We explore the classification performance of ZIPCWM, Fixed Zero-inflated Poisson mixture model (FZIP), and Poisson cluster weighted model (PCWM) on the data. Based on the confusion matrix, ZIPCWM achieves $97.4\%$ classification power, PCWM achieves $67.30\%$, while FZIP has the worst classification performance. In conclusion, ZIPCWM outperforms both PCWM and FZIP models.

==> biblio1.tex <==
@article{bilenko2004etal,
	title={Integrating constraints and metric learning in semi-supervised clustering.},
	author={Bilenko, S. and Mooney, J},
	journal = {\textit{International Conference on Machine Learning}},
	number={11},
	year={2004},
	volume = {1},
	publisher={ICML}
}

@article{xie2016etal,
	title={Unsupervised deep embedding for clustering analysis.},
	author={Xie, J, and Girshick, R and Farhadi, A.},
	journal = {\textit{International conference on machine learning}},
	number={478--487},
	volume = {1},
	year={2016},
	publisher={ACM}
}

@article{dempster1977etal,
	title={Maximum likelihood from incomplete data via the EM algorithm (with discussion)},
	author={Dempster, and A., and Laird and N., and Rubin and D.},
	number={1 - 38},
	journal = {\textit{Journal of the Royal Statistical Society, Series B}},
	volume = {1},
	year={1977},
	publisher={ACM}
}

@article{wu1983,
	title={On the convergence properties of the EM algorithm.},
	author={Wu, and J. F. J},
	journal = {\textit{The Annals of Statistics.}},
	volume = {11},
	number={1},
	pages = {95 -- 103},
	year={1983},
}

@article{vandePoletal1998,
	title={Propagation of probabilities, means and variances in mixed graphical association models.},
	author={Lauritzen, and S. and L},
	journal = {\textit{J American Statistical Association.}},
	volume = {1},
	number={1098--1108},
	year={1992},
}

@article{ueda2000,
	title={SMEM algorithm for mixture models.},
	author={Ueda, N. and Nakano, R. and Gharamani, Z. and Hinton, G},
	Journal = {\textit{Neural Computation}},
	volume = {12},
	number = {9},
	pages = {2109--2128},
	year={2000},
}


@article{vermuntandMagidson2000,
	title={Stochastic models, estimation and control, chapter 12.7.},
	journal = {\textit{Physics and Media Group, MIT Media Laboratory, Cambridge, Massachusetts 02139, USA.}},
	volume = {1},
	author={Maybeck P.S.},
	number={},
	year={1982},
}

@article{Bleietal2003,
	title={Hierarchical Bayesian Models for application in information retrieval.},
	author={Blei, D. M., and Jordan, M. I. and Ng, A. Y},
	journal = {\textit{Bayesian Statistics}},
	number={7},
	volume = {1},
	pages={25--43},
	year={2003},
	publisher={Oxford University Press}
}

@article{Forinaetal1986,
	title={Multivariate data analysis as a discriminating method of the origin of wines.},
	author={Forina, M., and Armanino, C., and Castino, M., and Ubigli, M.},
	number={3},
	journal = {\textit{Computational Statistics and Data Analysis,}},
	pages={189--201},
	volume = {25},
	year={1986},
	publisher={ACM}
}

@article{WilsonandMartinez2003,
	title={The general inefficiency of batch training for gradient descent learning.},
	author={Wilson, D. R. and Martinez, T. R},
	number={10},
	journal = {\textit{Neural Networks,}},
	pages={1429--1451. 279},
	volume = {16},
	year={2003},
	publisher={ACM}
}


@article{CeleuxandGovaert1995,
	title={Gaussian Parsimonious clustering models.},
	author={Celeux, G. and Govaert, G.},
	journal = { \textit{Pattern Recognition,}},
	volume = {28},
	number={5},
	pages={781--793},
	year={1995},
	publisher={ACM}
}

@article{CeleuxandGovaert1992,
	title={A classification EM algorithm for clustering and two stochastic versions.},
	author={Celeux, G. and Govaert, G.},
	journal = {\textit{Computational Statistics and Data Analysis,}},
	volume = {14},
	number={3},
	pages={315--332},
	year={1992},
	publisher={ACM}
}

@article{McLachlanandkrish1997,
	title={The EM Algorithm and Extentions.},
	author={McLachlan, G. and Krishnan, T.},
	journal = {\textit{New York,}},
	volume = {274},
	number={1},
	year={1997},
	publisher={ACM}
}

@article{FranzandDjamel2005,
	title={Genetic-Based EM Algorithm for Learning Gaussian Mixture Models},
	author={Franz, P., and Djamel, B.},
	journal = {\textit{IEEE Transactions on Pattern Analysis and Machine Iintelligence}},
	volume={27},
	number={8},
	year={2005},
	publisher={IEEE}
}

@article{MartinezandVitria2000,
	title={Learning mixture models using a genetic version of the EM algorithm.},
	author={Martınez, and A., and Vitria, and J.},
	journal = {\textit{Pattern Recognition Letters}},
	volume = {1},
	number={759--769},
	year={2000},
	publisher={ACM}
}

@article{MartinezandVitria2001,
	title={Clustering in image space for place recognition and visual annotations for human-robot interaction.},
	author={Martinez, A.M. and Vitria, J.},
	journal = {\textit{IEEE Trans. Systems Man Cybernet}, Cybernet.},
	volume = {Part-B, 31},
	number={5},
	pages={669--682},
	year={2001},
	publisher={ACM}
}

@article{Gershenfeldetal1999,
	title={Cluster-weighted modelling for time-series analysis.},
	author={Gershenfeld, and N., and Schoner, and B., and Metois, and E.},
	journal = {\textit{Physics and Media Group, MIT Media Laboratory, Cambridge, Massachusetts 02139, USA.}},
	number={1},
	volume = {1},
	year={1999},
	publisher={ACM}
}

@article{SchonerandGershenfeld2016,
	title={Cluster Weighted Models: Probabilistic Time Series Prediction, Characterization and Synthesis},
	author={Schoner, B. and Gershenfeld, N.},
	journal = {\textit{Physics and Media Group, MIT Media Laboratory, Cambridge, Massachusetts 02139, USA.}},
	volume = {1},
	number={1},
	year={2016},
	publisher={ACM}
}


@book{IanGoodfellowetal2015,
	title={Deep Learning.},
	author={Goodfellow, I and Bengio, Y. and Courville},
	number={1--787, series B},
	series = {B},
	year={2015},
	publisher={ACM}
}

@article{Ingrassiaetal2015,
	title={The generalized linear mixed cluster-weighted model.},
	author={Ingrassia, and S., and Punzo, and A., and Vittadini, and G., and Minotti, and S. C.},
	journal = {\textit{Journal of Classification}},
	volume = {32},
	number = {1},
	pages = {85 - 113},
	year={2015},
	publisher={ACM}
}

@article{Bertaetal2016,
	title={Multilevel cluster-weighted models for the evaluation of hospitals. },
	author={Berta, P., and Ingrassia, S., and Punzo, A., and Vittadini, G.},
	journal={\textit{DOI 10.1007/s40300-016-0098-3}},
	volume={2},
	number={74},
	pages={275--292},
	year={2016},
	publisher={ACM}
}

@article{Ingrassiaetal2012,
	title={Local statistical modeling via the cluster-weighted approach with eliptical  distributions.},
	author={Ingrassia, and S., and Punzo, and A., and Vittadini, and G., and Minotti, and S. C.,},
	journal={\textit{Journal of Classification} METRON},
	volume={29},
	number={3},
	pages={363--401},
	year={2012},
	publisher={ACM}
}

@article{Hennig2000,
	title={Identifiability of models for clusterwise linear regression.},
	author={Hennig, and C.},
	journal={\textit{Journal of classification}},
	volume={17},
	number={1},
	pages={237--296},
	year={2000},
	publisher={ACM}
}

@article{Ingrassiaetal2014,
	title={Model-based clustering via linear cluster-weighted models.},
	author={Ingrassia, and S., and Minotti, and S., and Punzo, A.},
	journal={\textit{Computational Statistics and Data Analysis,}},
	pages={159--182},
	number = {1},
	volume = {71},
	year={2014},
	publisher={ACM}
}

@article{MuthenandAsparouhov2009,
	title={Multilevel regression mxiture analysis.},
	author={Muthen, B and Asparouhov, T},
	journal={J. R. Stat. Soc. Ser. A (Stat. Soc.)},
	volume={3},
	number={172},
	pages={639--657},
	year={2009}
}

@article{Subedietal2012,
	title={Clustering and Classification via Cluster-Weighted Factor Analyzer},
	author={Subedi, S., and Punzo, A. and Ingrassia, S., and McNicholas, P.},
	journal={arXiv:1209.6463v1 [stat.ME]},
	volume={1},
	number={1},
	pages={1--36},
	year={2012}
}

@article{MengandVanDyk1997,
	title={The Expectation Maximization algorithm – an old folk-song sung to a fast new tune.},
	author={Meng, X. L. and D. van Dyk},
	journal={Journal of the Royal Statistical Society: Series B(Statistical Methodology)},
	volume={59},
	number={3},
	pages={511--567},
	year={1997},
	publisher={RSS}
}


@article{Punzo2012,
	title={Flexible Mixture Modeling with the Polynomial Gaussian Cluster-Weighted Model.},
	author={Antonio and P.,},
	journal={arXiv:1207.0939v1},
	volume={1},
	number={1},
	pages={1--25},
	year={2012},
	publisher={stat.ME}
}

@article{Guitierrezetal1995,
	title={Analysis of tomato root initiation using a normal mixture distribution.},
	author={Gutierrez, and R., and Carroll, R., and Wang, N., and Lee, G., and Taylor, B.},
	journal={Biometrics},
	volume={51},
	number={4},
	pages={1461--1468},
	year={1995},
	publisher={Taylor}
}


@article{Loetal2008, 
	title={Automated gating of flow cytometry data via robust model-based clustering.},
	author={Lo, K., and Brinkman, R., and Gottardo, R.},
	journal={Cytometry Part A},
	volume={73},
	number={4},
	pages={321--332},
	year={2008},
	publisher={ACM}
}

@article{AndersonEdgar1935,
	title={The irises of the Gaspe Peninsula.},
	author={Anderson, and E.},
	journal={Bulletin of the American Iris Society,},
	volume={Part II},
	number={59},
	pages={2–5.},
	year={1935},
	publisher={ACM}
}

@article{Fisher1936,
	title={The use of multiple measurements in taxonomic problems.},
	author={Fisher, and R. A.},
	journal={Annals of Eugenics,},
	volume={Part II},
	number={7},
	pages={179–188.},
	year={1936},
	publisher={Elsevier}
}


@article{Rosenblatt1958,
	title={The perceptron: a probability model for information storage and organization in the brain.},
	author={Rosenblatt, and F.},
	journal = {\textit{Psychological Review,}},
	volume={65},
	number={6},
	pages={386. 5},
	year={1958},
	publisher={ACM}
}


@article{Mahalanobis1930,
	title={On tests and measures of group divergence.},
	author={Mahalanobis, and P.C.},
	journal={\textit{Journal and Proceedings of the Asiatic Society of Bengal}},
	volume={Part I. Theoretical formulae.},
	number={26},
	pages={541--588. 5},
	year={1938},
	publisher={Proceeding}
}


@article{Fisher1938,
	title={The Statistical utilization of multiple measurements.},
	author={Fisher, and R. A.},
	journal={Annals of Human Genetics,},
	volume={8},
	number={4},
	pages={376--386. 5},
	year={1938},
	publisher={Genetics}
}

@article{Hotelling1931,
	title={The generalization of "Student's" ratio.},
	author={Hotelling, and H.},
	journal={\textit{Annals of Human Genetics,}},
	volume={1},
	number={5},
	pages={1},
	year={1931},
	publisher={Gentics}
}


@article{Cox1958,
	title={The generalization of "Student's" ratio.},
	author={Cox, and D. R.},
	journal={\textit{Journal of the Royal Statistical Society,}},
	volume={Series B (Methological)},
	number={5},
	pages={215--242},
	year={1958},
	publisher={RSS}
}


@article{chickandHeck1997,
	title={Tractable inference for complex stochastic processes.},
	author={Boyen, and X., and Koller, and D},
	journal = {\textit{Uncertainty in Al.}},
	number={1},
	volume = {1},
	year={1998},
	publisher = {ACM}
}

